Federated Dynamical Low-Rank Training with Global Loss Convergence Guarantees

In this work, we propose a federated dynamical low-rank training (FeDLRT) scheme to reduce client compute and communication costs - two significant performance bottlenecks in horizontal federated learning. Our method builds upon dynamical low-rank splitting schemes for manifold-constrained optimization to create a global low-rank basis of network weights, which enables client training on a small coefficient matrix. A consistent global low-rank basis allows us to incorporate a variance correction scheme and prove global loss descent and convergence to a stationary point. Dynamic augmentation and truncation of the low-rank bases automatically optimizes computing and communication resource utilization. We demonstrate the efficiency of FeDLRT in an array of computer vision benchmarks and show a reduction of client compute and communication costs by up to an order of magnitude with minimal impacts on global accuracy.

==> assets/algorithms/FeDLR.tex <==
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwComment{Comment}{$\triangleright$\ }{}


\Input{Initial low-rank factors $U,V\in\mathbb{R}^{n\times r}$ $\in\mathbb{R}^{r\times r}$;\\
{\tt adaptive}: Boolean flag that decides whether or not to dynamically update the ranks;\\
$\tau$: singular value threshold for the adaptive procedure.}
%
$U^{t=1}$, $S^{t=1}$, $V^{t=1}$ $\gets$ $U$, $S$, $V$ \tcc*{Initialization}
\For {$t=1,\dots, T$}{
$U_c$, $S_c$, $V_c$ $\gets$  $U^{t}$, $S^{t}$, $V^{t}$ $\quad\forall c\in C$ \tcc*{Broadcast to clients}
Compute $\nabla_U \mathcal{L}(U_cS_cV_c^{\top})$, and   $\nabla_V \mathcal{L}(U_c^{t}S_c^{t}V_c^{t,\top})$ $\quad\forall a\in C_a$ \tcc*{Basis gradient} 
$G_U\gets \sum_{c=1}^C q_c\nabla_U\mathcal{L}(U_cS_cV_c^{\top};X_c)$ \tcc*{Average client basis gradients}
$G_V\gets \sum_{c=1}^C q_c\nabla_V\mathcal{L}(U_cS_cV_c^{\top};X_c)$\\
$ [U \mid \Bar{U}] \gets  \mathrm{QR}([U \mid G_U])$ \tcc*{Augmentation and normaliztion on server}
$[V \mid \Bar{V}] \gets  \mathrm{QR}([V \mid G_V])$ \\% \tcc*{Augmentation and orthonormalization}
$\Bar{U}_c \gets \Bar{U}$ \tcc*{Broadcast to clients}
$\Bar{V}_c \gets \Bar{V}$ \\
$\widetilde{U}_c \gets [U_c\mid \Bar{U}_c]$  \tcc*{Client basis assembly}
$\widetilde{V}_c \gets [V_c\mid \Bar{V}_c]$ \\ 
$\widetilde{S}_c^{s=0}\gets \begin{bmatrix}
S_c & 0 \\
0 & 0
\end{bmatrix} $ \tcc*{Client coefficient matrix assembly}
\For(\tcc*[f]{Low-rank client training}){$s=1,\dots, t_*$}{
$\widetilde{S}_c^{s+1}\gets \widetilde{S}_c^{s} - \lambda \nabla_S\mathcal{L}(\widetilde{U}_c\widetilde{S}_c^{s}\widetilde{V}_c^\top)$\tcc*{Coefficient update on client}
}
$\widetilde{S}^*\gets  \sum_{c=1}^C q_c\widetilde{S}_c^{t_*}$ \tcc*{Average client coefficients}
\vspace{.5em}
$P_{r_1}, \Sigma_{r_1}, Q_{r_1} \gets$ SVD$(\widetilde{S}^*)$ with threshold  $\vartheta$ \tcc*{Compression step}
$U^{t+1}\gets   \widetilde{U}P_{r_1}$, and
$V^{t+1}\gets   \widetilde{V}Q_{r_1}$ \tcc*{Basis projection}
$S^{t+1}\gets \Sigma_{r_1}$ 
}


==> assets/algorithms/fl_dlrt_mk1.tex <==
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwComment{Comment}{$\triangleright$\ }{}


\Input{Initial low-rank factors $U,V\in\mathbb{R}^{n\times r}$ $\in\mathbb{R}^{r\times r}$;\\
{\tt adaptive}: Boolean flag that decides whether or not to dynamically update the ranks;\\
$\tau$: singular value threshold for the adaptive procedure.}
%
$U^{t=1}$, $S^{t=1}$, $V^{t=1}$ $\gets$ $U$, $S$, $V$ \tcc*{Initialization}
\For(\tcc*[f]{Global aggregation rounds}){$t=1,\dots, T$}{
Choose $C_a\subset C$\tcc*{Client selection}
$U_a^{l=1}$, $S_a^{l=1}$, $V_a^{l=1}$ $\gets$  $U^{t}$, $S^{t}$, $V^{t}$ $\quad\forall a\in C_a$ \tcc*{Broadcast to clients}
\For(\tcc*[f]{Low-rank client training}){$l=1,\dots, T_L$}{

%\mathcal{L}_a\gets \mathcal{L}(U_a^lS_a^lV_a^{l,\top})$ $\quad\forall a\in C_a$ \tcc*{Evaluation on clients}
Compute gradients $\nabla_U\mathcal{L}(U_a^l S_a^l V_a^{l,\top}; X_a)$, and   $\nabla_V\mathcal{L}(U_a^lS_a^lV_a^{l,\top}; X_a)$ $\quad\forall a\in C_a$\\ % \tcc*{Gradient tape eval. on clients} 
$\nabla_U\mathcal{L}_a\gets \nabla_U\mathcal{L}(U_a^l S_a^l V_a^{l,\top}; X_a)$ $\quad\forall a\in C_a$ \tcc*{Gradient computation}
$\nabla_V\mathcal{L}_a\gets \nabla_V\mathcal{L}(U_a^l S_a^l V_a^{l,\top}; X_a)$ $\quad\forall a\in C_a$\\% \tcc*{Computation on clients}



$U_a^{l+1}\gets \mathrm{QR}(U_a^t - \lambda  \nabla_{U}\mathcal{L}_a )$ \tcc*{Descend and orthonormalization}
$V_a^{l+1}\gets \mathrm{QR}(V_a^t - \lambda  \nabla_{V}\mathcal{L}_a )$ \\% \tcc*{Descend and orthonormalization}


$\widetilde{S}_a\gets  U_a^{{l+1},\top} U_a^t S_a^t V_a^{l,\top}V_a^{l+1}  $\tcc*{Projection onto new basis}


${S}_a^{l+1}\gets \widetilde{S}_a^{l} - \lambda \nabla_S\mathcal{L}(U_a^{l+1}\widetilde{S}_a^{l}V_a^{l+1, \top})$\tcc*{Coefficient update}
}
$W\gets  \sum_{a\in C_a}\frac{n_a}{n} U_a^{T_L} {S}_a^{T_L} V_a^{T_L,\top} $ \tcc*{Allreduce from $C_a$}
\vspace{.5em}

$U^{t+1}, S^{t+1},V^{t+1} \gets$ truncated SVD of $W$ with threshold  $\tau$ \tcc*{On server}

}


==> assets/algorithms/fl_dlrt_mk2.tex <==
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwComment{Comment}{$\triangleright$\ }{}


\Input{Initial low-rank factors $U,V\in\mathbb{R}^{n\times r}$ $\in\mathbb{R}^{r\times r}$;\\
{\tt adaptive}: Boolean flag that decides whether or not to dynamically update the ranks;\\
$\tau$: singular value threshold for the adaptive procedure.}
%
$U^{t=1}$, $S^{t=1}$, $V^{t=1}$ $\gets$ $U$, $S$, $V$ \tcc*{Initialization}
\For {$t=1,\dots, T$}{
Choose $C_a\subset C$\tcc*{Client selection}
$U_a^{t}$, $S_a^{t}$, $V_a^{t}$ $\gets$  $U^{t}$, $S^{t}$, $V^{t}$ $\quad\forall a\in C_a$ \tcc*{Broadcast to $C_a$}
$\mathcal{L}_a\gets \mathcal{L}(U_a^{t}S_a^{t}V_a^{t,\top})$ $\quad\forall a\in C_a$ \tcc*{Evaluation on clients}
Compute $\nabla_U\mathcal{L}_a$, and   $\nabla_V\mathcal{L}_a$ $\quad\forall a\in C_a$ \tcc*{Gradient tape eval. on clients} 

$\nabla_U\mathcal{L}\gets \sum_{a\in C_a}\frac{n_a}{n}\nabla_U\mathcal{L}_a$ \tcc*{Allreduce from $C_a$}
$\nabla_V\mathcal{L}\gets \sum_{a\in C_a}\frac{n_a}{n}\nabla_U\mathcal{L}_a$ \tcc*{Allreduce from $C_a$}

\If (\tcc*[f]{Basis augmentation step on server}){\tt adaptive} {
    $\widetilde{U},\_\gets  \mathrm{QR}([U \mid \nabla_{U}\mathcal{L}])$ \tcc*{Augmentation and orthonormalization}
    $\widetilde{V},\_\gets  \mathrm{QR}([V \mid \nabla_{V}\mathcal{L}])$ \\% \tcc*{Augmentation and orthonormalization}

}
\Else{
$\widetilde{U},\_\gets \mathrm{QR}(U - \lambda  \nabla_{U}\mathcal{L} )$ \tcc*{Descend and orthonormalization}
$\widetilde{V},\_\gets \mathrm{QR}(V - \lambda  \nabla_{V}\mathcal{L} )$ \\% \tcc*{Descend and orthonormalization}

}
$\widetilde{S}\gets  \widetilde{U}^\top U^t S^t V^{t,\top}\widetilde{V}  $\tcc*{Projection onto new basis on server}
$\widetilde{U}_a$, $\widetilde{S}_a^{l=0}$, $\widetilde{V}_a$ $\gets$  $\widetilde{U}$, $\widetilde{S}$, $\widetilde{V}$ $\quad\forall a\in C_a$ \tcc*{Broadcast to $C_a$}


\For(\tcc*[f]{Low-rank client training}){$l=1,\dots, T_L$}{
$\widetilde{S}_a^{l+1}\gets \widetilde{S}_a^{l} - \lambda \nabla_S\mathcal{L}(\widetilde{U}_a\widetilde{S}_a^{l}\widetilde{V}_a^\top)$\tcc*{Coefficient update on client}
}
$\widetilde{S}\gets  \sum_{a\in C_a}\frac{n_a}{n}\widetilde{S}_a^{T_L}$ \tcc*{Allreduce from $C_a$}
\vspace{.5em}

\If(\tcc*[f]{Rank adjustment step}){\tt adaptive}{
$P, S, Q \gets$ truncated SVD of $\widetilde{S}$ with singular value threshold  $\tau$\;
% \For {each mode $i$}{
$U\gets   \widetilde{U}P$, and
$V\gets   \widetilde{V}Q$ \\
% }
}\Else{
$U\gets \widetilde{U}$, and $V\gets \widetilde{V}$\\
}
}


==> assets/tables/backup.tex <==
\begin{NiceTabular}{l l | c c c c}[colortbl-like]
\toprule
  & Method stage & FeDLRT (simpl. var/cor) &  FedLin~\cite{NEURIPS2021_7a6bda9a} & FeDLR~\cite{qiao2021communicationefficient} & Riemannian FL~\cite{10146425}\\
\midrule
\multirow{3}{*}{{\rotatebox[origin=c]{90}{Client}}} & Basis gradient &  $\landauO(br(2n+4r))$ & n.a. & n.a. &$\landauO(2n^2r + 4n r^2 + 2nr)$  \\
                        & Variance correction & $\landauO(4r^2)$ & $\landauO(bn^2)$ & n.a. \\
                        & Client iteration & $\landauO(s_*2br(2n+2r))$  & $\landauO(s_*bn^2)$ & $\landauO(s_*bn^2 + n^3)$\\
\midrule
\multirow{4}{*}{{\rotatebox[origin=c]{90}{Server}}} & Gradient averaging & $\landauO(r(2n+4r))$ & $\landauO(n^2)$ & n.a. & $\landauO(2nr + n^2 r)$\\
                        & Basis augmentation & $\landauO(2nr^2)$ & n.a. & n.a. \\
                        & Aggregation & $\landauO(4r^2)$ & $\landauO(n^2)$ & $\landauO(n^2)$\\     
                        & Truncation & $\landauO((2r)^3)$ & n.a.  &  $\landauO(n^3)$ \\
\midrule
\multirow{4}{*}{{\rotatebox[origin=c]{90}{Bandwidth}}} 
 & Param. distribution & $\landauO(r(2n +r))$ & $\landauO(n^2)$ & $\landauO(2nr)$ &$\landauO(4nr)$\\
   & Basis \& var/cor (up) & $\landauO(r(2n +r))$ & $\landauO(n^2)$ & n.a. \\
& Aug. Basis \& var/cor (down) & $\landauO(r(2n +r))$ & $\landauO(n^2)$ & n.a \\
& Param. aggregation & $\landauO(4r^2)$ &  $\landauO(n^2)$ & $\landauO(2nr)$ \\
\bottomrule
\end{NiceTabular}
\\

==> assets/tables/experiments_object_detection.tex <==
 %\resizebox{0.48\textwidth}{!}
 {
\begin{NiceTabular}{ll| cc cc cc}
\toprule   
& &\multicolumn{2}{c}{VGG16}  & \multicolumn{2}{c}{Alexnet} & \multicolumn{2}{c}{ResNet18}\\
 \cmidrule{3-8}
& & test acc. [\%] & c.r. [\%] &  test acc. [\%] &c.r. [\%] & test acc. [\%] & c.r. [\%] \\ 
 %\cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} 
 \midrule
& Baseline
 &$89.43$ &$0.0$  &$85.46$ &$0.0$  &$94.33$ & $0.0$ \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{Low-rank}} &TDLRT  &  $\textbf{89.59}$ &$\textbf{95.34}$  &   $\textbf{82.39}$  & $\textbf{83.12}$ & $\textbf{92.72}$ & $78.73$  \\ 
& Matrix DLRT & $89.13 $ & $83.22$ & $73.57$ & $71.57$ &  $80.98$ &$56.85$ \\ 
% \midrule
&  Tucker-factorized & $83.74 $ & $61.34$ & $ 70.3$ & $69.74 $ & $ 91.11$ & $74.19$\\
&  Matrix-factorized & $79.96 $ & $87.20$ & $77.07 $ & { $68.20 $} &$92.07$  &{$77.49$}\\
&  CP-factorized & $83.68$ & {$78.85$} & $ 76.14$& {$ 71.46$} & $ 91.87$& {$ 69.95$} \\ 
 \midrule
%{Baseline (SNIP)}&$93.18$ &\multicolumn{2}{c}{$0.0$}  &$85.88$ &\multicolumn{2}{c}{$0$} &n.a. &\multicolumn{2}{c}{n.a.} \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{Pruning}} & {SNIP} & $89.58$ &{$56.23$}  &$-$ &{$-$} & $89.5$ & $78.5$ \\
& IMP & $87.21$ &{$58.54$}  &$-$ &{$-$} & $90.5$ & $\textbf{82.50}$ \\
& GraSP & $88.5$ &{$77.3$}  &$-$ &{$-$} & $89.4$ & $77.9$ \\
 \bottomrule
\end{NiceTabular}
}

==> assets/tables/tab_resnet18_cifar10.tex <==
 %\resizebox{\textwidth}{!}
 {
\begin{NiceTabular}{l| c c c c c c}
\toprule   
 \# clients & 1 &  2 & 4 & 8 & 12 \\
 \midrule
FedAvg &$94.47\pm 0.06$ &$93.31\pm 0.09$ & $90.93\pm 0.11$& $87.98\pm 0.07$ & $84.87\pm 0.10$ \\
FeDLRT, w/o var/cor &$94.55\pm 0.06$ &$93.12\pm 0.06$ & $91.13\pm 0.09$& $87.91\pm 0.07$ & $85.05\pm 0.09$ \\
\midrule
FedLin  \\
FeDLRT, var/cor \\
 \bottomrule
\end{NiceTabular}
}
% $89.14$ &{$95.0$}%

% \begin{NiceTabular}{|l|ccc|ccc|ccc|}
% \toprule   
% &\multicolumn{3}{c}{VGG16}  & \multicolumn{3}{c}{Alexnet} & \multicolumn{3}{c}{ResNet18}\\
%  \cmidrule{2-4}  \cmidrule{5-7}\cmidrule{8-10}
% &  & \multicolumn{2}{c}{compression rate [\%]} &  &\multicolumn{2}{c}{compression rate [\%]}&&\multicolumn{2}{c}{compression rate [\%]} \\ 
%  \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} 
%  method & test acc. [\%]  & eval & train & test acc. [\%]  & eval & train & test acc. [\%]  & eval & train\\ 
%  \midrule
% {Baseline}&$89.43$ &\multicolumn{2}{c}{$0.0$}  &$85.46$ &\multicolumn{2}{c}{$0$} &$94.33$ &\multicolumn{2}{c}{$0$} \\
% \midrule
% TDLRT  &  $\textbf{89.59}$ &$\textbf{95.34}$& $69.92$  &   $\textbf{82.39}$  & $\textbf{83.12}$ & $29.82$ & $\textbf{92.72}$ & $78.73$ & $50.80$ \\ 
% Matrix DLRT & $89.13 $ & $83.22$ & $74.30$ & $73.57$ & $71.57$ & $55.51$ & $80.98$ &$56.85$ &$13.71$ \\ 
% \midrule

%  Tucker-factorized & $83.74 $ & \multicolumn{2}{c}{$61.34$} & $ 70.3$ & \multicolumn{2}{c}{$69.74 $}& $ 91.11$ & \multicolumn{2}{c}{$74.19$}\\
%  Matrix-factorized & $79.96 $ & \multicolumn{2}{c}{$87.20$} & $77.07 $ & \multicolumn{2}{c}{ $68.20 $} &$92.07$  &\multicolumn{2}{c}{$77.49$}\\
%  CP-factorized & $83.68$ & \multicolumn{2}{c}{$78.85$} & $ 76.14$& \multicolumn{2}{c}{$ 71.46$} & $ 91.87$& \multicolumn{2}{c}{$ 69.95$} \\ 
%  \midrule
% %{Baseline (SNIP)}&$93.18$ &\multicolumn{2}{c}{$0.0$}  &$85.88$ &\multicolumn{2}{c}{$0$} &n.a. &\multicolumn{2}{c}{n.a.} \\
% {SNIP}&$89.14$ &\multicolumn{2}{c}{$95.0$}  &$84.59$ &\multicolumn{2}{c}{$90$} &n.a. &\multicolumn{2}{c}{n.a.} \\
%  \bottomrule
% \end{NiceTabular}
% }
\label{tab_cifar}
